PREMA: A Predictive Multi-task Scheduling Algorithm For Preemptible Neural Processing Units

To amortize cost, cloud vendors providing DNN acceleration as a service to end-users employ consolidation and virtualization to share the underlying resources among multiple DNN service requests. This paper makes a case for a "preemptible" neural processing unit (NPU) and a "predictive" multi-task scheduler to meet the latency demands of high-priority inference while maintaining high throughput. We evaluate both the mechanisms that enable NPUs to be preemptible and the policies that utilize them to meet scheduling objectives. We show that preemptive NPU multi-tasking can achieve an average 7.8x, 1.4x, and 4.8x improvement in latency, throughput, and SLA satisfaction, respectively.

==> IEEEtran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> tex/discussion.tex <==
\section{Discussion and Future Work}
\label{sect:discussion}

\begin{figure}[t!] \centering
\vspace{-0.5em}
	\includegraphics[width=0.43\textwidth]{./fig/IA_sparsity_vggnet.pdf}
\vspace{-0.5em}
\caption{
Changes in VGGNet's per-layer activation density during inference across $1000$ test images in ImageNet.
Similar observations were made for AlexNet/VGGNet but we omit the results due to space constraints.
}
\label{fig:ia_sparsity}
\end{figure}


{\bf Preemption with network sparsity.} There has been a large body of prior
work that explored the design of NPUs optimized for
sparsity~\cite{song:2015:eie,cnvlutin,cambriconx,stripes,bitpragmatic,intel:2017:icassp,intel:2017:fpga,whatmough:2017:isscc,whatmough:2017:hotchips,scnn,bittactical}.
As our work is the first that explores preemptive multi-tasking in NPUs, we
assumed the DNN models are dense and focused on preemption mechanisms
tailored for DNNs and the scheduling policies that utilizes them. As
discussed in \sect{sect:pred_model} however, a profile-based \proposed
predictor was shown to be highly effective in estimating the execution time of
a sparse-optimized NPU (e.g., SCNN), which leverages both activation and weight sparsity~\cite{scnn}.  The
reason behind its predictable execution time is twofold:
(1) weight sparsity is \emph{fixed} once pruned and retrained for deployment, so
the weight sparsity itself causes no variation in the execution time, (2) activation sparsity, which
is input data-dependent, was shown to exhibit small per-layer
variation at inference time.  \fig{fig:ia_sparsity} shows 
the changes in VGGNet's per-layer activation sparsity when profiled across
$1000$ ImageNet test images. As shown, the changes in activation density is
fairly low, causing small variation in the overall execution time. 








{\bf Preemptive multi-tasking under multi-NPU systems.} As DNNs
get more complex and deeper, ML practitioners
are seeking platforms that employ \emph{multiple} NPUs
within a system. For instance, NVIDIA's DGX-1~\cite{dgx_1v} as
well as Google's Cloud TPU employ multiple GPUs/TPUs per
node and the runtime system and the ML framework running on top of it 
provide parallelization solutions to split the DNN execution
across these multiple processors. As there exists multiple processing
engines under such multi-NPU context, the notion of preemptive multi-tasking
can be extended to \emph{spatial} multi-tasking beyond the
temporal multi-tasked NPU as explored in this paper. We leave
such exploration for future work.



==> tex/motivation.tex <==
\section{Motivation}
\label{sect:motivation}

\subsection{Why Preemptive Multi-tasking for NPUs?}
\label{sect:why_preemption}

Major cloud service vendors like Google, Amazon, and Microsoft currently deploy
several thousands of NPUs or GPUs in the datacenter to	provide DNN
acceleration as a \emph{service} to end-users (e.g., Google Cloud ML~\cite{google_cloud_ml},
		Amazon AMI~\cite{amazon_ami}, Azure ML~\cite{azure_ml}). To optimize
\todo{total-cost-of-ownership} of maintaining these warehouse-scale datacenters, cloud
service providers employ consolidation and virtualization as means to \emph{share}
the underlying hardware resources among \emph{multiple} DNN tasks. 
The key objective of our study is to enable flexible scheduling of multiple
inference service requests available on the NPU job scheduler via \emph{preemptive}
multitasking.  \fig{fig:why_preemption} shows how non-preemptive job scheduling
		algorithms are ineffective when a time-critical, high-priority inference
		task is competing with other low-priority tasks for the NPU compute
		resources.  \fig{fig:why_preemption}(a) shows the baseline, non-preemptive
		FCFS (first-come first-serve) scheduler where the high-priority task with a
		hard deadline (I3) is not able to be scheduled until the previously issued
		inference tasks (I1 and I2) have finished execution. A non-preemptive, but
		high-priority first scheduler (\fig{fig:why_preemption}(b)) can reduce the
		latency of I3 by prioritizing its execution over I2, but the latency reduction
		is marginal as it must be scheduled after I1's completion.  Because the
		execution time of I3 is dependent upon the previously issued I1 and I2's
		execution latency, it becomes challenging to satisfy the strong response-time
		demands of I3. As such, a \emph{preemption mechanism} that can
		proactively terminate low-priority tasks for high-priority ones to be able
		to be executed is required as illustrated through the example in
		\fig{fig:why_preemption}(c): I2 can finish earlier by preempting I1's execution
																 and I3 similarly preempts I1's execution, reducing
																 the average latency higher priority tasks (I2 and I3)
	experience. As more DNN inference services are offloaded
		and serviced from the cloud, a flexible yet intelligent scheduling algorithm
		for multi-tasked inference scenarios will be of utmost importance to satisfy 
		user responsiveness while maintaining fairness and system-level throughput.
		


